Learning Differential Equations that are Easy to Solve

Differential equations parameterized by neural networks become expensive to solve numerically as training progresses. We propose a remedy that encourages learned dynamics to be easier to solve. Specifically, we introduce a differentiable surrogate for the time cost of standard numerical solvers, using higher-order derivatives of solution trajectories. These derivatives are efficient to compute with Taylor-mode automatic differentiation. Optimizing this additional objective trades model performance against the time cost of solving the learned dynamics. We demonstrate our approach by training substantially faster, while nearly as accurate, models in supervised classification, density estimation, and time-series modelling tasks.

==> memes.tex <==
\section{Memes}

\subsection{Vince McMahon Reaction}

\texttt{jax.grad(jax.odeint(jax.jet(jax.neural\_net)))}

Do we also want \texttt{jax.vmap}?

\subsection{Sequel Transformation Speculation}

We have \texttt{jax.jit} and now \texttt{jax.jet}. What's next?

\texttt{jax.jat}
\begin{itemize}
\item ``just another transform''
\end{itemize}

\texttt{jax.jut}
\begin{itemize}
\item Appeal to ``jutting out'' as in getting snagged by jax's sharp bits.
\item Knife emoji
\end{itemize}

\texttt{jax.jot}
\begin{itemize}
\item quick, write that down
\end{itemize}

\texttt{jax.jyt}
\begin{itemize}
\item \begin{lstlisting}
def jax.jyt():
  return sometimes_even
\end{lstlisting}
\end{itemize}

\subsection{Pen Pineapple Apple Pen}

\begin{lstlisting}
I have a jax.jet, I have an jax.neural_net.
Uh! jax.jet(jax.neural_net)
I have a jax.grad, I have jax.odeint.
Uh! jax.grad(jax.odeint)
jax.jet(jax.neural_net)...
jax.jet(jax.odeint)...

jax.grad(jax.odeint(jax.jet(jax.neural_net)))!
\end{lstlisting}


Unfortunately the pen = pen symmetry is not preserved by jet = grad.
Possible deal breaker?

